A Hitchhiker's Guide On Distributed Training of Deep Neural Networks

Deep learning has led to tremendous advancements in the field of Artificial Intelligence. One caveat however is the substantial amount of compute needed to train these deep learning models. Training a benchmark dataset like ImageNet on a single machine with a modern GPU can take upto a week, distributing training on multiple machines has been observed to drastically bring this time down. Recent work has brought down ImageNet training time to a time as low as 4 minutes by using a cluster of 2048 GPUs. This paper surveys the various algorithms and techniques used to distribute training and presents the current state of the art for a modern distributed training framework. More specifically, we explore the synchronous and asynchronous variants of distributed Stochastic Gradient Descent, various All Reduce gradient aggregation strategies and best practices for obtaining higher throughout and lower latency over a cluster such as mixed precision training, large batch training and gradient compression.

==> bibliography.tex <==
@inproceedings{dean2012large,
  title={{Large scale distributed deep networks}},
  author={Dean, Jeffrey and Corrado, Greg and Monga, Rajat and Chen, Kai and Devin, Matthieu and Mao, Mark and Senior, Andrew and Tucker, Paul and Yang, Ke and Le, Quoc V and others},
  booktitle={Advances in neural information processing systems},
  pages={1223--1231},
  year={2012}
}

@article{jia2018highly,
  title={{Highly Scalable Deep Learning Training System with Mixed-Precision: Training ImageNet in Four Minutes}},
  author={Jia, Xianyan and Song, Shutao and He, Wei and Wang, Yangzihao and Rong, Haidong and Zhou, Feihu and Xie, Liqiang and Guo, Zhenyu and Yang, Yuanzhou and Yu, Liwei and others},
  journal={arXiv preprint arXiv:1807.11205},
  year={2018}
}

@article{goyal2017accurate,
  title={{Accurate, large minibatch SGD: training imagenet in 1 hour}},
  author={Goyal, Priya and Doll{\'a}r, Piotr and Girshick, Ross and Noordhuis, Pieter and Wesolowski, Lukasz and Kyrola, Aapo and Tulloch, Andrew and Jia, Yangqing and He, Kaiming},
  journal={arXiv preprint arXiv:1706.02677},
  year={2017}
}

@article{ginsburg2018large,
  title={{Large Batch Training of Convolutional Networks with Layer-wise Adaptive Rate Scaling}},
  author={Ginsburg, Boris and Gitman, Igor and You, Yang},
  year={2018}
}

@article{jin2016scale,
  title={{How to scale distributed deep learning?}},
  author={Jin, Peter H and Yuan, Qiaochu and Iandola, Forrest and Keutzer, Kurt},
  journal={arXiv preprint arXiv:1611.04581},
  year={2016}
}

@article{chen2016revisiting,
  title={{Revisiting distributed synchronous SGD}},
  author={Chen, Jianmin and Pan, Xinghao and Monga, Rajat and Bengio, Samy and Jozefowicz, Rafal},
  journal={arXiv preprint arXiv:1604.00981},
  year={2016}
}

@article{thakur2005optimization,
  title={{Optimization of collective communication operations in MPICH}},
  author={Thakur, Rajeev and Rabenseifner, Rolf and Gropp, William},
  journal={The International Journal of High Performance Computing Applications},
  volume={19},
  number={1},
  pages={49--66},
  year={2005},
  publisher={Sage Publications Sage CA: Thousand Oaks, CA}
}

@article{lin2017deep,
  title={{Deep gradient compression: Reducing the communication bandwidth for distributed training}},
  author={Lin, Yujun and Han, Song and Mao, Huizi and Wang, Yu and Dally, William J},
  journal={arXiv preprint arXiv:1712.01887},
  year={2017}
}

@article{micikevicius2017mixed,
  title={{Mixed precision training}},
  author={Micikevicius, Paulius and Narang, Sharan and Alben, Jonah and Diamos, Gregory and Elsen, Erich and Garcia, David and Ginsburg, Boris and Houston, Michael and Kuchaev, Oleksii and Venkatesh, Ganesh and others},
  journal={arXiv preprint arXiv:1710.03740},
  year={2017}
}

@inproceedings{abadi2016tensorflow,
  title={{Tensorflow: a system for large-scale machine learning.}},
  author={Abadi, Mart{\'\i}n and Barham, Paul and Chen, Jianmin and Chen, Zhifeng and Davis, Andy and Dean, Jeffrey and Devin, Matthieu and Ghemawat, Sanjay and Irving, Geoffrey and Isard, Michael and others},
  booktitle={OSDI},
  volume={16},
  pages={265--283},
  year={2016}
}

@article{akiba2017extremely,
  title={{Extremely large minibatch sgd: Training resnet-50 on imagenet in 15 minutes}},
  author={Akiba, Takuya and Suzuki, Shuji and Fukuda, Keisuke},
  journal={arXiv preprint arXiv:1711.04325},
  year={2017}
}

@inproceedings{deng2009imagenet,
  title={{Imagenet: A large-scale hierarchical image database}},
  author={Deng, Jia and Dong, Wei and Socher, Richard and Li, Li-Jia and Li, Kai and Fei-Fei, Li},
  booktitle={Computer Vision and Pattern Recognition, 2009. CVPR 2009. IEEE Conference on},
  pages={248--255},
  year={2009},
  organization={Ieee}
}

@techreport{gibiansky2017bringing,
  title={{Bringing HPC techniques to deep learning}},
  author={Gibiansky, Andrew},
  year={2017},
  institution={Baidu Research, Tech. Rep., 2017, http://research. baidu. com/bringing-hpc-techniques-deep-learning/. Bingjing Zhang TESTS \& CERTIFICATIONS IBM Certified Database Associate-DB2 Universal Database}
}

@article{smith2017don,
  title={{Don't Decay the Learning Rate, Increase the Batch Size}},
  author={Smith, Samuel L and Kindermans, Pieter-Jan and Le, Quoc V},
  journal={arXiv preprint arXiv:1711.00489},
  year={2017}
}

@article{sergeev2018horovod,
  title={{Horovod: fast and easy distributed deep learning in TensorFlow}},
  author={Sergeev, Alexander and Del Balso, Mike},
  journal={arXiv preprint arXiv:1802.05799},
  year={2018}
}

@inproceedings{krizhevsky2012imagenet,
  title={{Imagenet classification with deep convolutional neural networks}},
  author={Krizhevsky, Alex and Sutskever, Ilya and Hinton, Geoffrey E},
  booktitle={Advances in neural information processing systems},
  pages={1097--1105},
  year={2012}
}

@book{ghemawat2003google,
  title={{The Google file system}},
  author={Ghemawat, Sanjay and Gobioff, Howard and Leung, Shun-Tak},
  volume={37},
  number={5},
  year={2003},
  publisher={ACM}
}

@inproceedings{shvachko2010hadoop,
  title={{The hadoop distributed file system}},
  author={Shvachko, Konstantin and Kuang, Hairong and Radia, Sanjay and Chansler, Robert},
  booktitle={Mass storage systems and technologies (MSST), 2010 IEEE 26th symposium on},
  pages={1--10},
  year={2010},
  organization={Ieee}
}

@inproceedings{smith2017cyclical,
  title={{Cyclical learning rates for training neural networks}},
  author={Smith, Leslie N},
  booktitle={Applications of Computer Vision (WACV), 2017 IEEE Winter Conference on},
  pages={464--472},
  year={2017},
  organization={IEEE}
}

@article{jacob2017quantization,
  title={{Quantization and training of neural networks for efficient integer-arithmetic-only inference}},
  author={Jacob, Benoit and Kligys, Skirmantas and Chen, Bo and Zhu, Menglong and Tang, Matthew and Howard, Andrew and Adam, Hartwig and Kalenichenko, Dmitry}
}

@article{krishnamoorthi2018quantizing,
  title={{Quantizing deep convolutional networks for efficient inference: A whitepaper}},
  author={Krishnamoorthi, Raghuraman},
  journal={arXiv preprint arXiv:1806.08342},
  year={2018}
}

@misc{chahal_mathur_2018,
  title={{hydra-hoard/hydra}},
  url={https://github.com/hydra-hoard/hydra},
  journal={GitHub},
  author={Chahal, Karanbir and Mathur, Vaibhav},
  year={2018}
}

@article{mnih2013playing,
  title={{Playing atari with deep reinforcement learning}},
  author={Mnih, Volodymyr and Kavukcuoglu, Koray and Silver, David and Graves, Alex and Antonoglou, Ioannis and Wierstra, Daan and Riedmiller, Martin},
  journal={arXiv preprint arXiv:1312.5602},
  year={2013}
}

% repeated reference of alexnet

@article{devlin2018bert,
  title={{BERT: Pre-training of Deep Bidirectional Transformers for Language Understanding}},
  author={Devlin, Jacob and Chang, Ming-Wei and Lee, Kenton and Toutanova, Kristina},
  journal={arXiv preprint arXiv:1810.04805},
  year={2018}
}

@article{redmon2017yolo9000,
  title={{YOLO9000: better, faster, stronger}},
  author={Redmon, Joseph and Farhadi, Ali},
  journal={arXiv preprint},
  year={2017}
}

@article{kingma2014adam,
  title={{Adam: A method for stochastic optimization}},
  author={Kingma, Diederik P and Ba, Jimmy},
  journal={arXiv preprint arXiv:1412.6980},
  year={2014}
}

@article{tieleman2012lecture,
  title={{Lecture 6.5-rmsprop: Divide the gradient by a running average of its recent magnitude}},
  author={Tieleman, Tijmen and Hinton, Geoffrey},
  journal={COURSERA: Neural networks for machine learning},
  volume={4},
  number={2},
  pages={26--31},
  year={2012}
}

@incollection{bottou2010large,
  title={{Large-scale machine learning with stochastic gradient descent}},
  author={Bottou, L{\'e}on},
  booktitle={Proceedings of COMPSTAT'2010},
  pages={177--186},
  year={2010},
  publisher={Springer}
}

@article{ruder2016overview,
  title={{An overview of gradient descent optimization algorithms}},
  author={Ruder, Sebastian},
  journal={arXiv preprint arXiv:1609.04747},
  year={2016}
}

@inproceedings{zhang2014asynchronous,
  title={{Asynchronous distributed ADMM for consensus optimization}},
  author={Zhang, Ruiliang and Kwok, James},
  booktitle={International Conference on Machine Learning},
  pages={1701--1709},
  year={2014}
}

@inproceedings{li2013distributed,
  title={{Distributed delayed proximal gradient methods}},
  author={Li, Mu and Andersen, David G and Smola, Alexander},
  booktitle={NIPS Workshop on Optimization for Machine Learning},
  volume={3},
  pages={3},
  year={2013}
}

@inproceedings{johnson2013accelerating,
  title={{Accelerating stochastic gradient descent using predictive variance reduction}},
  author={Johnson, Rie and Zhang, Tong},
  booktitle={Advances in neural information processing systems},
  pages={315--323},
  year={2013}
}

@article{zhang2015staleness,
  title={{Staleness-aware async-sgd for distributed deep learning}},
  author={Zhang, Wei and Gupta, Suyog and Lian, Xiangru and Liu, Ji},
  journal={arXiv preprint arXiv:1511.05950},
  year={2015}
}

@article{zheng2016asynchronous,
  title={{Asynchronous stochastic gradient descent with delay compensation}},
  author={Zheng, Shuxin and Meng, Qi and Wang, Taifeng and Chen, Wei and Yu, Nenghai and Ma, Zhi-Ming and Liu, Tie-Yan},
  journal={arXiv preprint arXiv:1609.08326},
  year={2016}
}

@inproceedings{zhang2015deep,
  title={{Deep learning with elastic averaging SGD}},
  author={Zhang, Sixin and Choromanska, Anna E and LeCun, Yann},
  booktitle={Advances in Neural Information Processing Systems},
  pages={685--693},
  year={2015}
}

@techreport{krizhevsky2009learning,
  title={{Learning multiple layers of features from tiny images}},
  author={Krizhevsky, Alex},
  year={2009},
  institution={Citeseer}
}

@inproceedings{raft,
 author = {Ongaro, Diego and Ousterhout, John},
 title = {{In Search of an Understandable Consensus Algorithm}},
 booktitle = {Proceedings of the 2014 USENIX Conference on USENIX Annual Technical Conference},
 series = {USENIX ATC'14},
 year = {2014},
 isbn = {978-1-931971-10-2},
 location = {Philadelphia, PA},
 pages = {305--320},
 numpages = {16},
 url = {http://dl.acm.org/citation.cfm?id=2643634.2643666},
 acmid = {2643666},
 publisher = {USENIX Association},
 address = {Berkeley, CA, USA},
} 

@inproceedings{hunt2010zookeeper,
  title={{ZooKeeper: Wait-free Coordination for Internet-scale Systems.}},
  author={Hunt, Patrick and Konar, Mahadev and Junqueira, Flavio Paiva and Reed, Benjamin},
  booktitle={USENIX annual technical conference},
  volume={8},
  number={9},
  year={2010},
  organization={Boston, MA, USA}
}

@inproceedings{kreps2011kafka,
  title={{Kafka: A distributed messaging system for log processing}},
  author={Kreps, Jay and Narkhede, Neha and Rao, Jun and others},
  year={2011}
}

@article{lamport2001paxos,
  title={{Paxos made simple}},
  author={Lamport, Leslie and others},
  year={2001}
}

@inproceedings{chandra2007paxos,
  title={{Paxos made live: an engineering perspective}},
  author={Chandra, Tushar D and Griesemer, Robert and Redstone, Joshua},
  booktitle={Proceedings of the twenty-sixth annual ACM symposium on Principles of distributed computing},
  pages={398--407},
  year={2007},
  organization={ACM}
}

@article{lesliesuperconvergence,
  author    = {Leslie N. Smith},
  title     = {{A disciplined approach to neural network hyper-parameters: Part 1
               - learning rate, batch size, momentum, and weight decay}},
  journal   = {CoRR},
  volume    = {abs/1803.09820},
  year      = {2018},
  url       = {http://arxiv.org/abs/1803.09820},
  archivePrefix = {arXiv},
  eprint    = {1803.09820},
  timestamp = {Mon, 13 Aug 2018 16:46:45 +0200},
  biburl    = {https://dblp.org/rec/bib/journals/corr/abs-1803-09820},
  bibsource = {dblp computer science bibliography, https://dblp.org}
}

@InProceedings{resnet,
author = {He, Kaiming and Zhang, Xiangyu and Ren, Shaoqing and Sun, Jian},
title = {{Deep Residual Learning for Image Recognition}},
booktitle = {The IEEE Conference on Computer Vision and Pattern Recognition (CVPR)},
month = {June},
year = {2016}
}

@inproceedings{federated,
title	= {{Federated Learning: Strategies for Improving Communication Efficiency}},
author	= {Jakub Konečný and H. Brendan McMahan and Felix X. Yu and Peter Richtarik and Ananda Theertha Suresh and Dave Bacon},
year	= {2016},
URL	= {https://arxiv.org/abs/1610.05492},
booktitle	= {NIPS Workshop on Private Multi-Party Machine Learning}
}

@inproceedings{recht2011hogwild,
  title={{Hogwild: A lock-free approach to parallelizing stochastic gradient descent}},
  author={Recht, Benjamin and Re, Christopher and Wright, Stephen and Niu, Feng},
  booktitle={Advances in neural information processing systems},
  pages={693--701},
  year={2011}
}

@inproceedings{li2014communication,
  title={{Communication efficient distributed machine learning with the parameter server}},
  author={Li, Mu and Andersen, David G and Smola, Alexander J and Yu, Kai},
  booktitle={Advances in Neural Information Processing Systems},
  pages={19--27},
  year={2014}
}

@inproceedings{1bitsgd,
    author = {Seide, Frank and Fu, Hao and Droppo, Jasha and Li, Gang and Yu, Dong},
    title = {{1-Bit Stochastic Gradient Descent and Application to Data-Parallel Distributed Training of Speech DNNs}},
    booktitle = {Interspeech 2014},
    year = {2014},
    month = {September},
    edition = {Interspeech 2014}
}

@article{qsgd,
  author    = {Dan Alistarh and
               Jerry Li and
               Ryota Tomioka and
               Milan Vojnovic},
  title     = {{QSGD: Randomized Quantization for Communication-Optimal Stochastic
               Gradient Descent}},
  journal   = {CoRR},
  volume    = {abs/1610.02132},
  year      = {2016},
  url       = {http://arxiv.org/abs/1610.02132},
  archivePrefix = {arXiv},
  eprint    = {1610.02132},
  timestamp = {Mon, 13 Aug 2018 16:45:58 +0200},
  bibsource = {dblp computer science bibliography, https://dblp.org}
}

@article{greff2017lstm,
  title={{LSTM: A search space odyssey}},
  author={Greff, Klaus and Srivastava, Rupesh K and Koutn{\'\i}k, Jan and Steunebrink, Bas R and Schmidhuber, J{\"u}rgen},
  journal={IEEE transactions on neural networks and learning systems},
  volume={28},
  number={10},
  pages={2222--2232},
  year={2017},
  publisher={IEEE}
}

@inproceedings{wen2017terngrad,
  title={{Terngrad: Ternary gradients to reduce communication in distributed deep learning}},
  author={Wen, Wei and Xu, Cong and Yan, Feng and Wu, Chunpeng and Wang, Yandan and Chen, Yiran and Li, Hai},
  booktitle={Advances in neural information processing systems},
  pages={1509--1519},
  year={2017}
}

@inproceedings{Strom2015ScalableDD,
  title={{Scalable distributed DNN training using commodity GPU cloud computing}},
  author={Nikko Strom},
  booktitle={INTERSPEECH},
  year={2015}
}

@article{aji2017sparse,
  title={{Sparse communication for distributed gradient descent}},
  author={Aji, Alham Fikri and Heafield, Kenneth},
  journal={arXiv preprint arXiv:1704.05021},
  year={2017}
}

@inproceedings{dryden2016communication,
  title={{Communication quantization for data-parallel training of deep neural networks}},
  author={Dryden, Nikoli and Moon, Tim and Jacobs, Sam Ade and Van Essen, Brian},
  booktitle={Machine Learning in HPC Environments (MLHPC), Workshop on},
  pages={1--8},
  year={2016},
  organization={IEEE}
}

@article{chen2017adacomp,
  title={{AdaComp: Adaptive Residual Gradient Compression for Data-Parallel Distributed Training}},
  author={Chen, Chia-Yu and Choi, Jungwook and Brand, Daniel and Agrawal, Ankur and Zhang, Wei and Gopalakrishnan, Kailash},
  journal={arXiv preprint arXiv:1712.02679},
  year={2017}
}

@article{fbdata,
  title={{TechCrunch Article: 
How Big Is Facebook’s Data? 2.5 Billion Pieces Of Content And 500+ Terabytes Ingested Every Day}},
  author={Josh Constine},
  year={2012}
}
